Compositional Learning of Dynamical System Models Using Port-Hamiltonian Neural Networks

Many dynamical systems -- from robots interacting with their surroundings to large-scale multiphysics systems -- involve a number of interacting subsystems. Toward the objective of learning composite models of such systems from data, we present i) a framework for compositional neural networks, ii) algorithms to train these models, iii) a method to compose the learned models, iv) theoretical results that bound the error of the resulting composite models, and v) a method to learn the composition itself, when it is not known a priori. The end result is a modular approach to learning: neural network submodels are trained on trajectory data generated by relatively simple subsystems, and the dynamics of more complex composite systems are then predicted without requiring additional data generated by the composite systems themselves. We achieve this compositionality by representing the system of interest, as well as each of its subsystems, as a port-Hamiltonian neural network (PHNN) -- a class of neural ordinary differential equations that uses the port-Hamiltonian systems formulation as inductive bias. We compose collections of PHNNs by using the system's physics-informed interconnection structure, which may be known a priori, or may itself be learned from data. We demonstrate the novel capabilities of the proposed framework through numerical examples involving interacting spring-mass-damper systems. Models of these systems, which include nonlinear energy dissipation and control inputs, are learned independently. Accurate compositions are learned using an amount of training data that is negligible in comparison with that required to train a new model from scratch. Finally, we observe that the composite PHNNs enjoy properties of port-Hamiltonian systems, such as cyclo-passivity -- a property that is useful for control purposes.

==> figures/intro_figure/composite_trajectory.tex <==
\begin{axis}[
    anchor=west,
    x grid style={darkgray176},
    xticklabels={},
    xmin=0.0, xmax=6.0,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel={},
    ymin=-0.871643200516701, ymax=0.872202828526497,
    ytick style={color=black},
    yticklabels={},
    height=2.4cm,
    tick align=inside,
    width=3.5cm,
    ticks=none,
    % ymajorgrids,
    % xmajorgrids,
]

\addplot [ultra thick, compositeModelColor]
table {%
0 0.5
0.1 0.466337829828262
0.2 0.42577263712883
0.3 0.380290508270264
0.4 0.332071483135223
0.5 0.283249378204346
0.6 0.235743492841721
0.7 0.191521897912025
0.8 0.15238992869854
0.900000000000001 0.119078755378723
1 0.0934444442391396
1.1 0.0767307281494141
1.2 0.0698617845773697
1.3 0.0735516399145126
1.4 0.088058665394783
1.5 0.112281210720539
1.6 0.144749730825424
1.7 0.184949815273285
1.8 0.231022611260414
1.9 0.280849754810333
2 0.332263618707657
2.1 0.383710384368896
2.2 0.433530628681183
2.29999999999999 0.479139149188995
2.39999999999999 0.518893837928772
2.49999999999999 0.551259279251099
2.59999999999999 0.574757695198059
2.69999999999999 0.588324904441833
2.79999999999998 0.590519964694977
2.89999999999998 0.580017924308777
2.99999999999998 0.55623322725296
3.09999999999998 0.518159449100494
3.19999999999998 0.468531280755997
3.29999999999997 0.40872597694397
3.39999999999997 0.340833008289337
3.49999999999997 0.267439126968384
3.59999999999997 0.190864950418472
3.69999999999997 0.112773604691029
3.79999999999996 0.0345640555024147
3.89999999999996 -0.0419011898338795
3.99999999999996 -0.116496860980988
4.09999999999996 -0.188597559928894
4.19999999999995 -0.257994651794434
4.29999999999995 -0.324240565299988
4.39999999999995 -0.38696625828743
4.49999999999995 -0.445888459682465
4.59999999999995 -0.500744342803955
4.69999999999994 -0.551285207271576
4.79999999999994 -0.597267985343933
4.89999999999994 -0.638444483280182
4.99999999999994 -0.67454993724823
5.09999999999994 -0.705707669258118
5.19999999999993 -0.731343984603882
5.29999999999993 -0.750844419002533
5.39999999999993 -0.763750433921814
5.49999999999993 -0.769580721855164
5.59999999999993 -0.767884433269501
5.69999999999992 -0.758314430713654
5.79999999999992 -0.740880131721497
5.89999999999992 -0.716856479644775
5.99999999999992 -0.684995591640472
6.09999999999991 -0.645559668540955
6.19999999999991 -0.599596917629242
6.29999999999991 -0.547946035861969
6.39999999999991 -0.491582423448563
6.49999999999991 -0.431540161371231
6.5999999999999 -0.368838757276535
6.6999999999999 -0.304423809051514
6.7999999999999 -0.239130884408951
6.8999999999999 -0.173670917749405
6.9999999999999 -0.108631402254105
7.09999999999989 -0.0444895029067993
7.19999999999989 0.0183902494609356
7.29999999999989 0.0797449350357056
7.39999999999989 0.139310479164124
7.49999999999988 0.196852266788483
7.59999999999988 0.252157151699066
7.69999999999988 0.304457098245621
7.79999999999988 0.354048818349838
7.89999999999988 0.400825053453445
7.99999999999987 0.444572687149048
8.09999999999987 0.485059827566147
8.19999999999987 0.522031009197235
8.29999999999987 0.555202484130859
8.39999999999987 0.584258198738098
8.49999999999986 0.609738111495972
8.59999999999986 0.629533886909485
8.69999999999986 0.643739104270935
8.79999999999986 0.652269423007965
8.89999999999985 0.654669284820557
8.99999999999985 0.650495827198029
9.09999999999985 0.639352560043335
9.19999999999985 0.620932579040527
9.29999999999985 0.595073938369751
9.39999999999984 0.561824381351471
9.49999999999984 0.521496117115021
9.59999999999984 0.475077033042908
9.69999999999984 0.423100799322128
9.79999999999984 0.366294890642166
9.89999999999983 0.305789232254028
};

\addplot [ultra thick, compositeModelColor]
table {%
0 -0.200000002980232
0.1 -0.148818999528885
0.2 -0.0789146050810814
0.3 0.00600391533225775
0.4 0.101603552699089
0.5 0.203627347946167
0.6 0.307239264249802
0.7 0.408394783735275
0.8 0.503380954265594
0.900000000000001 0.588933348655701
1 0.662179887294769
1.1 0.720594584941864
1.2 0.76324862241745
1.3 0.787694811820984
1.4 0.792364120483398
1.5 0.774346172809601
1.6 0.735464215278625
1.7 0.677410960197449
1.8 0.602354645729065
1.9 0.513281285762787
2 0.413031578063965
2.1 0.305133551359177
2.2 0.193209528923035
2.29999999999999 0.0820893794298172
2.39999999999999 -0.0258367415517569
2.49999999999999 -0.127796694636345
2.59999999999999 -0.221131861209869
2.69999999999999 -0.305435031652451
2.79999999999998 -0.377666682004929
2.89999999999998 -0.437576502561569
2.99999999999998 -0.480759978294373
3.09999999999998 -0.508072435855865
3.19999999999998 -0.521593153476715
3.29999999999997 -0.522954225540161
3.39999999999997 -0.514480590820312
3.49999999999997 -0.4995396733284
3.59999999999997 -0.480319231748581
3.69999999999997 -0.458778917789459
3.79999999999996 -0.436354547739029
3.89999999999996 -0.413235187530518
3.99999999999996 -0.389952659606934
4.09999999999996 -0.369078874588013
4.19999999999995 -0.349444687366486
4.29999999999995 -0.331039726734161
4.39999999999995 -0.313749760389328
4.49999999999995 -0.297389507293701
4.59999999999995 -0.281726539134979
4.69999999999994 -0.266497105360031
4.79999999999994 -0.251116275787354
4.89999999999994 -0.235456302762032
4.99999999999994 -0.219632118940353
5.09999999999994 -0.203311860561371
5.19999999999993 -0.186144545674324
5.29999999999993 -0.167791962623596
5.39999999999993 -0.147527307271957
5.49999999999993 -0.12552572786808
5.59999999999993 -0.102415435016155
5.69999999999992 -0.0785214155912399
5.79999999999992 -0.053452804684639
5.89999999999992 -0.0273095741868019
5.99999999999992 -0.00170863908715546
6.09999999999991 0.0227629635483027
6.19999999999991 0.045672133564949
6.29999999999991 0.0667772367596626
6.39999999999991 0.0860115811228752
6.49999999999991 0.103436291217804
6.5999999999999 0.119189336895943
6.6999999999999 0.13344033062458
6.7999999999999 0.146362468600273
6.8999999999999 0.158111467957497
6.9999999999999 0.168813705444336
7.09999999999989 0.178559795022011
7.19999999999989 0.187756240367889
7.29999999999989 0.196901649236679
7.39999999999989 0.205079644918442
7.49999999999988 0.212140172719955
7.59999999999988 0.217908620834351
7.69999999999988 0.221791848540306
7.79999999999988 0.223906278610229
7.89999999999988 0.224133089184761
7.99999999999987 0.222217470407486
8.09999999999987 0.217899888753891
8.19999999999987 0.211644992232323
8.29999999999987 0.203398242592812
8.39999999999987 0.191729545593262
8.49999999999986 0.176363855600357
8.59999999999986 0.157124504446983
8.69999999999986 0.133995354175568
8.79999999999986 0.10717785358429
8.89999999999985 0.0771218910813332
8.99999999999985 0.0445301830768585
9.09999999999985 0.0103452755138278
9.19999999999985 -0.024290943518281
9.29999999999985 -0.0580081380903721
9.39999999999984 -0.0886470824480057
9.49999999999984 -0.116429068148136
9.59999999999984 -0.140757665038109
9.69999999999984 -0.161419883370399
9.79999999999984 -0.178544268012047
9.89999999999983 -0.192494839429855
};

\addplot [ultra thick, compositeModelColor, dashed]
table {%
0 -0.300000011920929
0.1 -0.377693384885788
0.2 -0.436854630708694
0.3 -0.47478723526001
0.4 -0.490593433380127
0.5 -0.485035330057144
0.6 -0.459807455539703
0.7 -0.417607754468918
0.8 -0.360632032155991
0.900000000000001 -0.290547013282776
1 -0.20834344625473
1.1 -0.116307258605957
1.2 -0.0166519619524479
1.3 0.0875274017453194
1.4 0.191868484020233
1.5 0.290793806314468
1.6 0.378206342458725
1.7 0.448602139949799
1.8 0.498578548431396
1.9 0.525197863578796
2 0.530097484588623
2.1 0.51436710357666
2.2 0.479909926652908
2.29999999999999 0.428470134735107
2.39999999999999 0.361324489116669
2.49999999999999 0.279269456863403
2.59999999999999 0.182863518595695
2.69999999999999 0.0729034841060638
2.79999999999998 -0.0489869341254234
2.89999999999998 -0.179522156715393
2.99999999999998 -0.313119232654572
3.09999999999998 -0.441741675138474
3.19999999999998 -0.556205034255981
3.29999999999997 -0.650205314159393
3.39999999999997 -0.716461777687073
3.49999999999997 -0.759514033794403
3.59999999999997 -0.781620740890503
3.69999999999997 -0.787133991718292
3.79999999999996 -0.780202746391296
3.89999999999996 -0.764127850532532
3.99999999999996 -0.741358637809753
4.09999999999996 -0.713661432266235
4.19999999999995 -0.682226419448853
4.29999999999995 -0.647799730300903
4.39999999999995 -0.610834181308746
4.49999999999995 -0.571521997451782
4.59999999999995 -0.529904723167419
4.69999999999994 -0.485897541046143
4.79999999999994 -0.439319133758545
4.89999999999994 -0.389944523572922
4.99999999999994 -0.337499916553497
5.09999999999994 -0.281716078519821
5.19999999999993 -0.222337901592255
5.29999999999993 -0.159153833985329
5.39999999999993 -0.0920485407114029
5.49999999999993 -0.0210775826126337
5.59999999999993 0.0534145794808865
5.69999999999992 0.131464347243309
5.79999999999992 0.211401909589767
5.89999999999992 0.290610074996948
5.99999999999992 0.365427166223526
6.09999999999991 0.434867650270462
6.19999999999991 0.49656680226326
6.29999999999991 0.548732936382294
6.39999999999991 0.590422332286835
6.49999999999991 0.621569514274597
6.5999999999999 0.642814755439758
6.6999999999999 0.655250549316406
6.7999999999999 0.660147309303284
6.8999999999999 0.658758163452148
6.9999999999999 0.652217388153076
7.09999999999989 0.641457676887512
7.19999999999989 0.627225518226624
7.29999999999989 0.609710454940796
7.39999999999989 0.589685380458832
7.49999999999988 0.567556142807007
7.59999999999988 0.543492794036865
7.69999999999988 0.517562329769135
7.79999999999988 0.489764332771301
7.89999999999988 0.460032403469086
7.99999999999987 0.428217440843582
8.09999999999987 0.394123464822769
8.19999999999987 0.357921093702316
8.29999999999987 0.31938511133194
8.39999999999987 0.276183485984802
8.49999999999986 0.229143753647804
8.59999999999986 0.178465589880943
8.69999999999986 0.123506858944893
8.79999999999986 0.0631420612335205
8.89999999999985 -0.00268427841365337
8.99999999999985 -0.0732724666595459
9.09999999999985 -0.147822558879852
9.19999999999985 -0.22307762503624
9.29999999999985 -0.2984299659729
9.39999999999984 -0.371749252080917
9.49999999999984 -0.440146297216415
9.59999999999984 -0.500897467136383
9.69999999999984 -0.551926732063293
9.79999999999984 -0.592724204063416
9.89999999999983 -0.624288201332092
};

\addplot [ultra thick, compositeModelColor, dashed]
table {%
0 0.100000001490116
0.1 0.224909499287605
0.2 0.337080538272858
0.3 0.430532276630402
0.4 0.500838696956635
0.5 0.546344339847565
0.6 0.567416250705719
0.7 0.56528103351593
0.8 0.544273257255554
0.900000000000001 0.506608963012695
1 0.454539000988007
1.1 0.389555305242538
1.2 0.312879353761673
1.3 0.22554224729538
1.4 0.128668621182442
1.5 0.0238106492906809
1.6 -0.0867417678236961
1.7 -0.19970591366291
1.8 -0.310737460851669
1.9 -0.414718061685562
2 -0.506556510925293
2.1 -0.582307159900665
2.2 -0.640057444572449
2.29999999999999 -0.6800616979599
2.39999999999999 -0.704216063022614
2.49999999999999 -0.715257346630096
2.59999999999999 -0.716090381145477
2.69999999999999 -0.709432601928711
2.79999999999998 -0.697630167007446
2.89999999999998 -0.682641446590424
2.99999999999998 -0.666078627109528
3.09999999999998 -0.64862447977066
3.19999999999998 -0.632231414318085
3.29999999999997 -0.617237329483032
3.39999999999997 -0.603889644145966
3.49999999999997 -0.592062294483185
3.59999999999997 -0.580929756164551
3.69999999999997 -0.569975256919861
3.79999999999996 -0.558854281902313
3.89999999999996 -0.54686963558197
3.99999999999996 -0.533079206943512
4.09999999999996 -0.516822040081024
4.19999999999995 -0.497504562139511
4.29999999999995 -0.474599331617355
4.39999999999995 -0.447727888822556
4.49999999999995 -0.417328983545303
4.59999999999995 -0.382104307413101
4.69999999999994 -0.341580450534821
4.79999999999994 -0.295413672924042
4.89999999999994 -0.243312209844589
4.99999999999994 -0.185056865215302
5.09999999999994 -0.120713375508785
5.19999999999993 -0.0500495918095112
5.29999999999993 0.026697114109993
5.39999999999993 0.108890630304813
5.49999999999993 0.195210665464401
5.59999999999993 0.283958286046982
5.69999999999992 0.372590005397797
5.79999999999992 0.457877606153488
5.89999999999992 0.53642863035202
5.99999999999992 0.605419397354126
6.09999999999991 0.663080394268036
6.19999999999991 0.708869814872742
6.29999999999991 0.743259906768799
6.39999999999991 0.767374217510223
6.49999999999991 0.782558977603912
6.5999999999999 0.790148854255676
6.6999999999999 0.791281700134277
6.7999999999999 0.786862134933472
6.8999999999999 0.777554988861084
6.9999999999999 0.763860583305359
7.09999999999989 0.746074736118317
7.19999999999989 0.724395573139191
7.29999999999989 0.698926329612732
7.39999999999989 0.669698476791382
7.49999999999988 0.636711776256561
7.59999999999988 0.600192606449127
7.69999999999988 0.5595982670784
7.79999999999988 0.514683246612549
7.89999999999988 0.465166598558426
7.99999999999987 0.410712391138077
8.09999999999987 0.350949198007584
8.19999999999987 0.285505920648575
8.29999999999987 0.214058741927147
8.39999999999987 0.136426523327827
8.49999999999986 0.0527348928153515
8.59999999999986 -0.0363718792796135
8.69999999999986 -0.128641486167908
8.79999999999986 -0.222484514117241
8.89999999999985 -0.315409511327744
8.99999999999985 -0.404372483491898
9.09999999999985 -0.48624175786972
9.19999999999985 -0.558193445205688
9.29999999999985 -0.620366275310516
9.39999999999984 -0.670050978660583
9.49999999999984 -0.707190930843353
9.59999999999984 -0.732903122901917
9.69999999999984 -0.748750448226929
9.79999999999984 -0.755287706851959
9.89999999999983 -0.753997385501862
};

\end{axis}

==> figures/intro_figure/submodel1_trajectory.tex <==
\begin{axis}[
    anchor=north,
    x grid style={darkgray176},
    xticklabels={},
    xmin=0.0, xmax=10.0,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel={},
    ymin=-0.553117728233337, ymax=0.550148463249207,
    ytick style={color=black},
    yticklabels={},
    height=2.3cm,
    tick align=inside,
    width=3cm,
    ticks=none,
    % ymajorgrids,
    % xmajorgrids,
]
\addplot [ultra thick, submodel1Color, solid]
table {%
0 0.5
0.1 0.467425584793091
0.2 0.429951995611191
0.3 0.388341397047043
0.4 0.343414485454559
0.5 0.296051114797592
0.6 0.247032627463341
0.7 0.197110131382942
0.8 0.1469596773386
0.900000000000001 0.0971766412258148
1 0.0482780598104
1.1 0.000710333231836557
1.2 -0.0451602339744568
1.3 -0.0890133902430534
1.4 -0.130523964762688
1.5 -0.169398158788681
1.6 -0.205370336771011
1.7 -0.238199949264526
1.8 -0.267668575048447
1.9 -0.293583512306213
2 -0.315762460231781
2.1 -0.334445297718048
2.2 -0.348480552434921
2.29999999999999 -0.358299136161804
2.39999999999999 -0.364068329334259
2.49999999999999 -0.365500330924988
2.59999999999999 -0.362575203180313
2.69999999999999 -0.354834645986557
2.79999999999998 -0.342730045318604
2.89999999999998 -0.326543986797333
2.99999999999998 -0.30661016702652
3.09999999999998 -0.283610075712204
3.19999999999998 -0.257466346025467
3.29999999999997 -0.228600069880486
3.39999999999997 -0.197464823722839
3.49999999999997 -0.164532661437988
3.59999999999997 -0.130280926823616
3.69999999999997 -0.0951811522245407
3.79999999999996 -0.0596898607909679
3.89999999999996 -0.0242418851703405
3.99999999999996 0.0107538681477308
4.09999999999996 0.0449162758886814
4.19999999999995 0.0778928846120834
4.29999999999995 0.109358355402946
4.39999999999995 0.139014229178429
4.49999999999995 0.166586980223656
4.59999999999995 0.191826730966568
4.69999999999994 0.214506193995476
4.79999999999994 0.234420746564865
4.89999999999994 0.25138857960701
4.99999999999994 0.265252351760864
5.09999999999994 0.275881409645081
5.19999999999993 0.283174067735672
5.29999999999993 0.287060916423798
5.39999999999993 0.287507981061935
5.49999999999993 0.284519791603088
5.59999999999993 0.278142392635345
5.69999999999992 0.268465638160706
5.79999999999992 0.255327254533768
5.89999999999992 0.23957072198391
5.99999999999992 0.221032872796059
6.09999999999991 0.199981927871704
6.19999999999991 0.176721826195717
6.29999999999991 0.151584967970848
6.39999999999991 0.124923951923847
6.49999999999991 0.0971032381057739
6.5999999999999 0.0684913322329521
6.6999999999999 0.0394537225365639
6.7999999999999 0.0103471083566546
6.8999999999999 -0.0184851698577404
6.9999999999999 -0.0467162355780602
7.09999999999989 -0.0740380212664604
7.19999999999989 -0.100162617862225
7.29999999999989 -0.12482276558876
7.39999999999989 -0.147772163152695
7.49999999999988 -0.1687853038311
7.59999999999988 -0.187657371163368
7.69999999999988 -0.204204246401787
7.79999999999988 -0.218262627720833
7.89999999999988 -0.229690790176392
7.99999999999987 -0.238370001316071
8.09999999999987 -0.244206219911575
8.19999999999987 -0.247133120894432
8.29999999999987 -0.246851146221161
8.39999999999987 -0.242890551686287
8.49999999999986 -0.236293017864227
8.59999999999986 -0.22687728703022
8.69999999999986 -0.215290173888206
8.79999999999986 -0.20126773416996
8.89999999999985 -0.184875413775444
8.99999999999985 -0.166345179080963
9.09999999999985 -0.145938754081726
9.19999999999985 -0.123941421508789
9.29999999999985 -0.100655518472195
9.39999999999984 -0.076393723487854
9.49999999999984 -0.0514732524752617
9.59999999999984 -0.026210144162178
9.69999999999984 -0.000914860051125288
9.79999999999984 0.0241115521639585
9.89999999999983 0.0485804118216038
};
% \addlegendentry{q predicted}
\addplot [ultra thick, submodel1Color, dashed]
table {%
0 -0.300000011920929
0.1 -0.352255970239639
0.2 -0.397263318300247
0.3 -0.434307962656021
0.4 -0.463040053844452
0.5 -0.483552753925323
0.6 -0.496287405490875
0.7 -0.501891493797302
0.8 -0.501188457012177
0.900000000000001 -0.494961977005005
1 -0.483875602483749
1.1 -0.468559890985489
1.2 -0.44954639673233
1.3 -0.427266955375671
1.4 -0.401906132698059
1.5 -0.373830109834671
1.6 -0.34331950545311
1.7 -0.310668170452118
1.8 -0.276194423437119
1.9 -0.239589557051659
2 -0.200886562466621
2.1 -0.160483568906784
2.2 -0.118664048612118
2.29999999999999 -0.0760251134634018
2.39999999999999 -0.0326314307749271
2.49999999999999 0.0110952332615852
2.59999999999999 0.0546533167362213
2.69999999999999 0.0974659621715546
2.79999999999998 0.138895273208618
2.89999999999998 0.178267002105713
2.99999999999998 0.214904963970184
3.09999999999998 0.248171761631966
3.19999999999998 0.277511686086655
3.29999999999997 0.302486568689346
3.39999999999997 0.322797000408173
3.49999999999997 0.338292688131332
3.59999999999997 0.348963379859924
3.69999999999997 0.35493415594101
3.79999999999996 0.356697767972946
3.89999999999996 0.354214638471603
3.99999999999996 0.347740560770035
4.09999999999996 0.336929351091385
4.19999999999995 0.32273867726326
4.29999999999995 0.305607378482819
4.39999999999995 0.285898953676224
4.49999999999995 0.263745129108429
4.59999999999995 0.239402666687965
4.69999999999994 0.212934866547585
4.79999999999994 0.184554606676102
4.89999999999994 0.154480636119843
4.99999999999994 0.122945994138718
5.09999999999994 0.0902072787284851
5.19999999999993 0.0565524362027645
5.29999999999993 0.0223071277141571
5.39999999999993 -0.012161641381681
5.49999999999993 -0.0464457720518112
5.59999999999993 -0.0801007971167564
5.69999999999992 -0.112655863165855
5.79999999999992 -0.143628612160683
5.89999999999992 -0.172544538974762
5.99999999999992 -0.198958083987236
6.09999999999991 -0.222474336624146
6.19999999999991 -0.242766603827477
6.29999999999991 -0.259590476751328
6.39999999999991 -0.272789031267166
6.49999999999991 -0.282330453395844
6.5999999999999 -0.288374811410904
6.6999999999999 -0.290775537490845
6.7999999999999 -0.289653480052948
6.8999999999999 -0.285172909498215
6.9999999999999 -0.276851505041122
7.09999999999989 -0.266007721424103
7.19999999999989 -0.252563536167145
7.29999999999989 -0.236694395542145
7.39999999999989 -0.218454286456108
7.49999999999988 -0.198088228702545
7.59999999999988 -0.175791412591934
7.69999999999988 -0.151762276887894
7.79999999999988 -0.126207619905472
7.89999999999988 -0.0993486195802689
7.99999999999987 -0.0713258311152458
8.09999999999987 -0.0423860736191273
8.19999999999987 -0.0129391187801957
8.29999999999987 0.0166816972196102
8.39999999999987 0.0461137108504772
8.49999999999986 0.0749709978699684
8.59999999999986 0.102853745222092
8.69999999999986 0.129360482096672
8.79999999999986 0.15410178899765
8.89999999999985 0.176715135574341
8.99999999999985 0.196878388524055
9.09999999999985 0.214321449398994
9.19999999999985 0.228834852576256
9.29999999999985 0.241113513708115
9.39999999999984 0.248675718903542
9.49999999999984 0.253661185503006
9.59999999999984 0.255357593297958
9.69999999999984 0.252498120069504
9.79999999999984 0.247731402516365
9.89999999999983 0.240411430597305
};
    
    
\end{axis}

==> figures/intro_figure/submodel2_trajectory.tex <==
\begin{axis}[
    anchor=north,
    x grid style={darkgray176},
    xticklabels={},
    xmin=0.0, xmax=10.0,
    xtick style={color=black},
    y grid style={darkgray176},
    ylabel={},
    ymin=-1.07771412432194, ymax=1.07858417332172,
    ytick style={color=black},
    yticklabels={},
    height=2.3cm,
    tick align=inside,
    width=3cm,
    ticks=none,
    % ymajorgrids,
    % xmajorgrids,
]

\addplot [ultra thick, submodel2Color]
table {%
0 0.5
0.1 0.471542656421661
0.2 0.446228116750717
0.3 0.424208372831345
0.4 0.405509740114212
0.5 0.390031367540359
0.6 0.377547770738602
0.7 0.367710024118423
0.8 0.360053271055222
0.900000000000001 0.354006767272949
1 0.348907589912415
1.1 0.344017446041107
1.2 0.338541626930237
1.3 0.33167976140976
1.4 0.322641015052795
1.5 0.310498088598251
1.6 0.294470280408859
1.7 0.273870408535004
1.8 0.248145237565041
1.9 0.216907054185867
2 0.179951816797256
2.1 0.13726644217968
2.2 0.089037612080574
2.29999999999999 0.0356584563851357
2.39999999999999 -0.0222815368324518
2.49999999999999 -0.0842322334647179
2.59999999999999 -0.14914844930172
2.69999999999999 -0.216103002429008
2.79999999999998 -0.284232437610626
2.89999999999998 -0.353429049253464
2.99999999999998 -0.422002702951431
3.09999999999998 -0.489071786403656
3.19999999999998 -0.554497480392456
3.29999999999997 -0.617527782917023
3.39999999999997 -0.677634179592133
3.49999999999997 -0.734250545501709
3.59999999999997 -0.786746680736542
3.69999999999997 -0.834465861320496
3.79999999999996 -0.876720368862152
3.89999999999996 -0.912793219089508
3.99999999999996 -0.941935539245605
4.09999999999996 -0.963360548019409
4.19999999999995 -0.976189494132996
4.29999999999995 -0.978178203105927
4.39999999999995 -0.970676064491272
4.49999999999995 -0.952231764793396
4.59999999999995 -0.921630322933197
4.69999999999994 -0.878825128078461
4.79999999999994 -0.823838591575623
4.89999999999994 -0.758980512619019
4.99999999999994 -0.687256634235382
5.09999999999994 -0.608435988426208
5.19999999999993 -0.524601221084595
5.29999999999993 -0.437549084424973
5.39999999999993 -0.348549664020538
5.49999999999993 -0.259167045354843
5.59999999999993 -0.169736355543137
5.69999999999992 -0.0807136222720146
5.79999999999992 0.0074203833937645
5.89999999999992 0.0942422226071358
5.99999999999992 0.179363384842873
6.09999999999991 0.262421280145645
6.19999999999991 0.343068540096283
6.29999999999991 0.420965939760208
6.39999999999991 0.495775073766708
6.49999999999991 0.567148923873901
6.5999999999999 0.634935677051544
6.6999999999999 0.69859391450882
6.7999999999999 0.757514297962189
6.8999999999999 0.811104357242584
6.9999999999999 0.858694732189178
7.09999999999989 0.899551689624786
7.19999999999989 0.932892441749573
7.29999999999989 0.958143293857574
7.39999999999989 0.974349141120911
7.49999999999988 0.980477511882782
7.59999999999988 0.97503250837326
7.69999999999988 0.957481622695923
7.79999999999988 0.927442252635956
7.89999999999988 0.884927928447723
7.99999999999987 0.830553710460663
8.09999999999987 0.765578508377075
8.19999999999987 0.691798090934753
8.29999999999987 0.611250579357147
8.39999999999987 0.525901913642883
8.49999999999986 0.437436819076538
8.59999999999986 0.347205013036728
8.69999999999986 0.256239742040634
8.79999999999986 0.16532476246357
8.89999999999985 0.0750597715377808
8.99999999999985 -0.0140767171978951
9.09999999999985 -0.101682014763355
9.19999999999985 -0.187398016452789
9.29999999999985 -0.270889431238174
9.39999999999984 -0.35275736451149
9.49999999999984 -0.432068169116974
9.59999999999984 -0.507299065589905
9.69999999999984 -0.578687965869904
9.79999999999984 -0.646112561225891
9.89999999999983 -0.709109365940094
};
% \addlegendentry{q predicted}
\addplot [ultra thick, submodel2Color, dashed]
table {%
0 -0.300000011920929
0.1 -0.269181698560715
0.2 -0.236325338482857
0.3 -0.202714279294014
0.4 -0.169611603021622
0.5 -0.138260185718536
0.6 -0.109873309731483
0.7 -0.0856146812438965
0.8 -0.0665690004825592
0.900000000000001 -0.0537091866135597
1 -0.0478638149797916
1.1 -0.0496881529688835
1.2 -0.0596398077905178
1.3 -0.0777987688779831
1.4 -0.104256972670555
1.5 -0.138763785362244
1.6 -0.180741995573044
1.7 -0.229267284274101
1.8 -0.283026069402695
1.9 -0.340293973684311
2 -0.398962646722794
2.1 -0.456659525632858
2.2 -0.510957181453705
2.29999999999999 -0.559659063816071
2.39999999999999 -0.601056337356567
2.49999999999999 -0.634097576141357
2.59999999999999 -0.658812522888184
2.69999999999999 -0.674511253833771
2.79999999999998 -0.681786119937897
2.89999999999998 -0.681471765041351
2.99999999999998 -0.674136579036713
3.09999999999998 -0.660258769989014
3.19999999999998 -0.640442192554474
3.29999999999997 -0.614733219146729
3.39999999999997 -0.583040714263916
3.49999999999997 -0.545278370380402
3.59999999999997 -0.501225113868713
3.69999999999997 -0.450525552034378
3.79999999999996 -0.392701417207718
3.89999999999996 -0.326656997203827
3.99999999999996 -0.253240764141083
4.09999999999996 -0.170746609568596
4.19999999999995 -0.0788864269852638
4.29999999999995 0.0230398569256067
4.39999999999995 0.132956296205521
4.49999999999995 0.249164626002312
4.59999999999995 0.36680880188942
4.69999999999994 0.482332319021225
4.79999999999994 0.589975237846375
4.89999999999994 0.683729469776154
4.99999999999994 0.758982062339783
5.09999999999994 0.815136909484863
5.19999999999993 0.853984534740448
5.29999999999993 0.878504574298859
5.39999999999993 0.89201158285141
5.49999999999993 0.896978497505188
5.59999999999993 0.894644975662231
5.69999999999992 0.887301206588745
5.79999999999992 0.875872135162354
5.89999999999992 0.860662698745728
5.99999999999992 0.841964602470398
6.09999999999991 0.819966316223145
6.19999999999991 0.794579863548279
6.29999999999991 0.765716254711151
6.39999999999991 0.733303844928741
6.49999999999991 0.697070240974426
6.5999999999999 0.656673073768616
6.6999999999999 0.611705720424652
6.7999999999999 0.561655819416046
6.8999999999999 0.505865037441254
6.9999999999999 0.443570911884308
7.09999999999989 0.373900473117828
7.19999999999989 0.295826494693756
7.29999999999989 0.208177715539932
7.39999999999989 0.110749050974846
7.49999999999988 0.00332161597907543
7.59999999999988 -0.113477475941181
7.69999999999988 -0.237023234367371
7.79999999999988 -0.363312095403671
7.89999999999988 -0.486622899770737
7.99999999999987 -0.599912583827972
8.09999999999987 -0.696964383125305
8.19999999999987 -0.774250626564026
8.29999999999987 -0.83144998550415
8.39999999999987 -0.870557427406311
8.49999999999986 -0.894708096981049
8.59999999999986 -0.907071232795715
8.69999999999986 -0.910397946834564
8.79999999999986 -0.906792104244232
8.89999999999985 -0.897757709026337
8.99999999999985 -0.884357452392578
9.09999999999985 -0.867158710956573
9.19999999999985 -0.846531808376312
9.29999999999985 -0.822627425193787
9.39999999999984 -0.795436680316925
9.49999999999984 -0.76481032371521
9.59999999999984 -0.730512797832489
9.69999999999984 -0.692216396331787
9.79999999999984 -0.64952427148819
9.89999999999983 -0.601971387863159
};

\end{axis}
